MV-Datalog+-: Effective Rule-based Reasoning with Uncertain Observations

Modern applications combine information from a great variety of sources. Oftentimes, some of these sources, like Machine-Learning systems, are not strictly binary but associated with some degree of (lack of) confidence in the observation. We propose MV-Datalog and MV-Datalog+- as extensions of Datalog and Datalog+-, respectively, to the fuzzy semantics of infinite-valued Lukasiewicz logic L as languages for effectively reasoning in scenarios where such uncertain observations occur. We show that the semantics of MV-Datalog exhibits similar model-theoretic properties as Datalog. In particular, we show that (fuzzy) entailment can be decided via minimal fuzzy models. We show that when they exist, such minimal fuzzy models are unique (when they exist) and can be characterised in terms of a linear optimisation problem over the output of a fixed-point procedure. On the basis of this characterisation, we propose similar many-valued semantics for rules with existential quantification in the head, extending Datalog+-. This paper is under consideration for acceptance in TPLP.

==> app.tex <==

\subsection{Implementation}
\todo[inline]{Pseudo-code,Explanation}

\subsection{Applications}
\todo[inline]{Add application examples if we have space (probably not).}
\subsection{Experiments}
Number of potential generated varying amount of certain facts\\
Time needed for potential generation and cumulative time inference + potential + MAP inference



==> make_arxiv.tex <==
#!/bin/sh

mkdir -p arxiv
cp 0-main.bbl arxiv/main.bbl
cp macros.sty tlparxiv.cls arxiv/
#cp graphics/nswex_new.pdf graphics/hierarchy.pdf graphics/fptex.pdf graphics/cneg_example.pdf arxiv/graphics/

#mkdir -p arxiv/figs
#cp figs/H0.pdf figs/nphard_ghd.pdf arxiv/figs/

# remove comments (except empty) and mash into one file
# latexpand in texlive-extra-utils ubuntu package or at https://www.ctan.org/pkg/latexpand
latexpand --empty-comments 0-main.tex > arxiv/main.tex



